Video Description: A Survey of Methods, Datasets and Evaluation Metrics

Video description is the automatic generation of natural language sentences that describe the contents of a given video. It has applications in human-robot interaction, helping the visually impaired and video subtitling. The past few years have seen a surge of research in this area due to the unprecedented success of deep learning in computer vision and natural language processing. Numerous methods, datasets and evaluation metrics have been proposed in the literature, calling the need for a comprehensive survey to focus research efforts in this flourishing new direction. This paper fills the gap by surveying the state of the art approaches with a focus on deep learning models; comparing benchmark datasets in terms of their domains, number of classes, and repository size; and identifying the pros and cons of various evaluation metrics like SPICE, CIDEr, ROUGE, BLEU, METEOR, and WMD. Classical video description approaches combined subject, object and verb detection with template based language models to generate sentences. However, the release of large datasets revealed that these methods can not cope with the diversity in unconstrained open domain videos. Classical approaches were followed by a very short era of statistical methods which were soon replaced with deep learning, the current state of the art in video description. Our survey shows that despite the fast-paced developments, video description research is still in its infancy due to the following reasons. Analysis of video description models is challenging because it is difficult to ascertain the contributions, towards accuracy or errors, of the visual features and the adopted language model in the final description. Existing datasets neither contain adequate visual diversity nor complexity of linguistic structures. Finally, current evaluation metrics ...

==> Datasets.tex <==
% Table generated by Excel2LaTeX from sheet 'Datasets'
\begin{table*}[h!]
\setlength\extrarowheight{2.5pt}
\small
\setlength\tabcolsep{2pt}
\centering
\caption{Standard datasets for benchmarking video description methods.}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
%\begin{tabularx}{\textwidth}{@{}l*{10}{C}@{}} (Eliminate the vertical whitespace before the first column and after the final column)
\noalign{\hrule height 1.15 pt}
    \hline
    \multicolumn{1}{|c|}{\textbf{Dataset}} & \textbf{Domain} & \multicolumn{1}{m{3.2em}|}{\textbf{No of\newline{classes}}} & \multicolumn{1}{m{3.2em}|}{\textbf{No of\newline{} Videos}} & \multicolumn{1}{m{3.2em}|}{\textbf{Avg\newline{} Length }} & \multicolumn{1}{m{3.2em}|}{\textbf{No of\newline{} Clips}} & \multicolumn{1}{m{4.2em}|}{\textbf{No of\newline{} Sentences}} & \multicolumn{1}{m{3.2em}|}{\textbf{No of\newline{} Words}} & \textbf{Vocab} & \multicolumn{1}{m{3.2em}|}{\textbf{Length\newline{}(Hrs)}}\\
    \hline
%     KTH \cite{schuldt2004recognizing} & {Human} & 6 & 2,391 & {-} & 2,391 & - & - & - & - \\
%     \hline
%     Lapt\& Perz \cite{laptev2007retrieving} & {Drink/Smoke} & - & - & - & - & - & - & - & - \\
%     \hline
%     Hollywood 2 \cite{marszalek2009actions} & Movie  & - & 4,000 & 20 sec & - & - & - & - & - \\
%     \hline
%     HMDB 51 \cite{kuehne2011hmdb} & Movie & 51 & 7,000 & 3 sec & - & - & - & - & - \\
%     \hline
    MSVD \cite{chen2011collecting} & Open (YTube) & 218 & 1970 & 10 sec & 1,970 & 70,028 & 607,339 & 13,010 & 5.30\\
    \hline
%     UCF50 \cite{reddy2013recognizing} & Human & 50 & - & - & - & - & - & - & - \\
%     \hline
%     UCF101 \cite{soomro2012ucf101} & Sports & 101 & 13,320 & 7 sec & - & - & - & - & 27.00 \\
%     \hline
    MPII Cooking \cite{rohrbach2012database} & Cooking & 65 & 44 & 600 sec & - & 5,609 & - & - & 8 \\
    \hline
    YouCook \cite{das2013thousand} & Cooking (YTube) & 6 & 88 & - & Nil & 2,688 & 42,457 & 2,711 & 2.30 \\
    \hline
%     KITTI \cite{geiger2013vision} & Driving & 1 & 21 & 30 sec & - & 520   & - & - & - \\
%     \hline
    TACoS \cite{regneri2013grounding} & Cooking & 26 & 127 & 360 sec & 7,206 & 18,227 & 146,771 & 28,292 & 15.9 \\
    \hline
%     Sports 1M \cite{karpathy2014large}& Sports & 500 & 1.1M & 300 sec & - & - & - & - & - \\
%     \hline
    TACos-MLevel \cite{rohrbach2014coherent}& Cooking & 1 & 185 & 360 sec & 14,105 & 52,593 & 2,000 & - & 27.1 \\
    \hline
%     Thumos 15 \cite{gorban2015thumos}& Sports & - & 21,000 & 4 sec & - & - & - & - & - \\
%     \hline
%     ActivityNet \cite{caba2015activitynet} & Human & - & 20,000 & 180 sec & - & - & - & - & - \\
%     \hline
    MPII-MD \cite{rohrbach2015dataset} & Movie & - & 94 & 3.9 sec & 68,337 & 68,375 & 653,467 & 24,549 & 73.60 \\
    \hline
    M-VAD \cite{torabi2015using} & Movie & - & 92 & 6.2 sec & 48,986 & 55,904 & 519,933 & 17,609 & 84.60 \\
    \hline
    MSR-VTT \cite{xu2016msr} & {Open} & 20 & 7,180 & 20 sec & 10,000 & 200,000 & 1,856,523 & 29,316 & 41.20 \\
    \hline
    Charades \cite{sigurdsson2016hollywood} & Human & 157 & 9,848 & 30 sec & - & 27,847 & - & - & 82.01 \\
    \hline
%     TGIF \cite{li2016tgif} & {Open} & - & 100,000 & 30 sec & 100,000 & 125,781 & - & - & 86.10 \\
%     \hline
    VTW \cite{zeng2016generation} & {Open} (YTube) & - & 18,100 & 90 sec & - & 44,613 & - & - & 213.20 \\
    \hline
    ActyNet Cap \cite{krishna2017dense} & Open & - & 20,000 & 180 sec & - & 100,000 & 1,348,000 & - & 849.00 \\
    \hline
%     \textcolor{red}{LSMDC} \cite{rohrbach2017movie} & Open  & - & 200 & - & - & 128,000 & - & - & 150.00 \\
%     \hline
\end{tabular}
\label{tab:datasets}
\end{table*}

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************

